D2.3 Power models, energy models and libraries for energy-efficient concurrent data structures and algorithms

This deliverable reports the results of the power models, energy models and libraries for energy-efficient concurrent data structures and algorithms as available by project month 30 of Work Package 2 (WP2). It reports i) the latest results of Task 2.2-2.4 on providing programming abstractions and libraries for developing energy-efficient data structures and algorithms and ii) the improved results of Task 2.1 on investigating and modeling the trade-off between energy and performance of concurrent data structures and algorithms. The work has been conducted on two main EXCESS platforms: Intel platforms with recent Intel multicore CPUs and Movidius Myriad platforms.

==> temp/Myriad-power-models-0.tex <==
This section presents the improvements on power models for Myriad1 platform from the model proposed in Deliverable D2.2.
\remind{cite the myriad1 architecture in Deliverable D1.1 and the previous version of power model D2.2}
The study is summarized to three main works as follows.
\begin{itemize}
\item We propose new application-general fine-grained power models (namely, RTHpower) that provide insights into how a given application consumes power when running on an ultra-low power embedded system. The RTHpower models consider three parameter groups: platform properties, application properties (e.g. operational intensity and scalability) and execution settings (e.g., the number of cores executing a given application). 
The models consider both platform and application properties, which give more insights into how to design applications to achieve better energy efficiency. (cf. Section \ref{sec:PowerModel}) 
\item We train the new RTHpower models on an ultra-low power embedded system, namely Movidius Myriad using different sets of micro-benchmarks and validate the models using two computation kernels from Berkeley dwarfs \cite{Asa06} and one data-intensive kernel from Graph500 benchmarks \cite{6114175}. The three chosen application kernels are dense matrix multiplication (Matmul), sparse matrix vector multiplication (SpMV) and breadth first search (BFS). The model fitting has percentage error at most 7\% for  micro-benchmarks and the model accuracy is 10\% for application benchmarks (cf. Section \ref{sec:Validation}). 
\item We investigate the RTH strategy on an ultra-low power embedded platform using the new RTHpower models. We propose a framework that is able to predict precisely when to and when not to apply the RTH strategy in order to minimize energy consumption. We validate the framework using micro-benchmarks and application kernels. From our experiments, we show real scenarios when to use RTH and when not to use RTH. We can save up to 61\% energy for dense matrix multiplication, 59\% energy for SpMV by using RTH and up to 5\% energy for BFS by not using RTH. (cf. Section \ref{sec:Framework})
\end{itemize}

\subsubsection{RTHpower - Analytical Power Models}
\label{sec:PowerModel}
We first present a new power model for operation units and then develop it to the RTHpower models considering application properties.
\paragraph{Power Model for Operation Units}
The experimental results of the micro-benchmarks suite for operation units show that the power consumption of Movidius Myriad platform is ruled by Equation \ref{eq:Pfirst}. In the equation, the static power $P^{sta}$ is the needed power when the Myriad chip is on, including memory storage power; the active power $P^{act}$ is the power consumed when a SHAVE core is on and actively performing computation work; the dynamic power $P^{dyn}(op)$ is the power consumed by each operation unit such as arithmetic units (e.g., IAU, VAU, SAU, CMU) or load/store units (e.g., LSU0, LSU1) in one SHAVE.  The experimental results show that different operation units have different $P^{dyn}(op)$ values as listed in Table~\ref{table:Punits}. Total dynamic power of a SHAVE core is the sum of all dynamic power from involved units. If benchmarks or programs are executed with $n$ SHAVE cores, the active and dynamic power needs to be multiplied with the number of used SHAVE cores. By using regression techniques, the average value of $P^{sta}$ and $P^{act}$ from all micro-benchmarks are computed in Equation \ref{eq:Pstat1} and Equation \ref{eq:Pstat2}. Table \ref{table:Parameters} provides the description of parameters in the proposed models. 
\begin{equation} \label{eq:Pfirst}
	P^{units}=P^{sta}+ n \times \left(P^{act} + \sum_i{P^{dyn}_i(op)} \right)
\end{equation}
\begin{equation} \label{eq:Pstat1}
	P^{sta}=61.81 \text{ mW}
\end{equation}
\begin{equation} \label{eq:Pstat2}
	P^{act}=29.33 \text{ mW}
\end{equation}
\begin{table}
\caption{\textbf{$P^{dyn}(op)$} of SHAVE Operation Units}
\label{table:Punits}
\begin{center}
\begin{tabular}{lll}
\hline\noalign{\smallskip}
Operation & Description & $P^{dyn}$ (mW)\\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
SAUXOR  &  Perform bitwise exclusive-OR on scalar              & 14.68          \\ 
SAUMUL  &  Perform scalar multiplication               & 17.69          \\ 
VAUXOR  &  Perform bitwise exclusive-OR on vector               & 34.34         \\
VAUMUL  &  Perform vector multiplication             & 51.98         \\ 
IAUXOR  &  Perform bitwise exclusive-OR on integer              & 15.91          \\ 
IAUMUL  &  Perform integer multiplication              & 18.48          \\ 
CMUCPSS &  Copy scalar to scalar             & 12.62          \\ 
CMUCPIVR&  Copy integer to vector              & 18.84         \\ 
LSULOAD &  Load from a memory address to a register            & 29.87         \\ 
LSUSTORE&  Store from a register to a memory address              & 37.49          \\
\noalign{\smallskip}\hline
\end{tabular}
\end{center}
\end{table}
\begin{table}
\caption{Model Parameter List}
\label{table:Parameters}
\begin{center}
\begin{tabular}{ll}
\hline\noalign{\smallskip}
Parameter & Description \\
\noalign{\smallskip}\hline\noalign{\smallskip}
$P^{sta}$                & Static power of a whole chip         \\ 
$P^{act}$                 & Active power of a core        \\ 
$P^{dyn}(op)$                  & Dynamic power of an operation unit        \\ 
$P^{LSU}$                  & Dynamic power of Load Store Unit          \\ 
$P^{ctn}$                  & Contention power of a core waiting for data          \\ 
$m$                 & Average number of active cores accessing data       \\ 
$n$                & Number of assigned cores to the program      \\ 
$I$              & Operational intensity of an application         \\ 
$\alpha$                & Time ratio of data transfer to computation       \\
$\beta$ & Communication pattern of an application\\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}
\paragraph{RTHpower Models for Applications}
\label{sec:ModelEquation}
Since typical applications require both computation and data movement, we use the concept of operational intensity proposed by Williams et al.\cite{Williams2009} to characterize applications. An application can be characterized by the amount of computational work $W$ and data transfer $Q$. $W$ is the number of operations performed by an application. $Q$ is the number of transferred bytes required during the program execution. Both $W$ and $Q$ define the operational intensity $I$ of applications as in Equation \ref{eq:PIWQ}. 
\begin{equation} \label{eq:PIWQ}
	I= \frac{W}{Q}
\end{equation}
As the time required to perform one operation is different from the time required to transfer one byte of data, we introduce a parameter to the models: time ratio {$\alpha$} of transferring one byte of data to performing one arithmetic operation. Ratio {$\alpha$} is the property of an application on a specific platform and its value depends on the application. 
 
Since the time to access data and time to perform computation work can be overlapped, during a program execution, the SHAVE core can be in one of the three states: performing computation, performing data transfer or performing both computation and data transfer in parallel. An application either has data transfer time longer than computation time or vice versa. Therefore, there are two models for the two cases. 

If data transfer time is longer than computation time, the model follows Equation \ref{eq:PalbiWQ}. The execution can be modeled as two (composed) periods: one is when computation and data transfer are performed in parallel and the other is when only data transfer is performed. Fraction $\frac{W}{\alpha \times Q}$ represents the overlapped time of computation and data transfer. Fraction $\frac{\alpha \times Q-W}{\alpha \times Q}$ represents the remaining time for data transfer. 

If computation time is longer than data transfer time, estimated power follows Equation \ref{eq:PalleWQ}. The execution can be modeled as two periods: one is when computation and data transfer are performed in parallel and the other is when only computation is performed.
\begin{equation} 
\label{eq:PalbiWQ} 
\begin{split}
	P&= P^{comp||data} \times (\frac{W}{\alpha \times Q})+  P^{data} \times (\frac{\alpha \times Q-W}{\alpha \times Q})
\end{split}
\end{equation}
\begin{equation} 
\label{eq:PalleWQ} 
\begin{split}
	P&= P^{comp||data} \times (\frac{\alpha \times Q}{W}) + P^{comp} \times (\frac{W-\alpha \times Q}{W})
\end{split}
\end{equation}
After converting W and Q to I by using Equation ~\ref{eq:PIWQ}, the final models are simplified as Equation \ref{eq:PalbiI} and Equation \ref{eq:PalleI},
\begin{equation} 
\label{eq:PalbiI} 
\begin{split}
	P&= P^{comp||data} \times (\frac{I}{\alpha})+  P^{data} \times (\frac{\alpha-I}{\alpha})
\end{split}
\end{equation}
\begin{equation} 
\label{eq:PalleI} 
\begin{split}
	P&= P^{comp||data} \times (\frac{\alpha}{I}) + P^{comp} \times (\frac{I-\alpha}{I})
\end{split}
\end{equation}
where $P^{data}$, $P^{comp}$ and $P^{comp||data}$ are explained below:

\textbf{Data transfer power $P^{data}$}: $P^{data}$ is the power consumed by the whole chip when only data transfer is performed. $P^{data}$ is computed by Equation \ref{eq:Pdata}. In Equation \ref{eq:Pdata}, $P^{sta}$ is the static power; $P^{act}$ is the active power; $n$ is the number of active cores assigned to run the application;  $m$ is the average number of SHAVE cores accessing data in parallel during the application execution; contention power $P^{ctn}$ is the power overhead occurring when a SHAVE core waits for accessing data because of the limited memory ports (or bandwidth) or cache size in the platform architecture. Therefore, $n-m$ is the average number of SHAVE cores waiting for memory access during the application execution. 
\begin{equation} \label{eq:Pdata}
\begin{split}
	P^{data} &= P^{sta} + min(m,n) \times (P^{act}+ P^{LSU})\\
	&+ max(n-m, 0) \times P^{ctn} 
\end{split}
\end{equation}
\textbf{Computation power $P^{comp}$}: $P^{comp}$ is the power consumed by the whole chip when only computation is performed. $P^{comp}$ is computed by Equation \ref{eq:Pcomp}. Each core runs its arithmetic units (e.g. IAU, SAU, VAU) to perform computation work. There is no contention power due to no memory access. Therefore, all assigned cores are active and contribute to total power.
\begin{equation} 
\label{eq:Pcomp} 
\begin{split}
	P^{comp}&= P^{sta} + n \times (P^{act}+\sum_i{P^{dyn}_i(op)})
\end{split}
\end{equation}
\textbf{Computation and data transfer power $P^{comp||data}$}: $P^{comp||data}$ is the power consumed by the whole chip when computation and data transfer are performed in parallel. $P^{comp||data}$ is computed by Equation \ref{eq:Pcompdata}. In this case, there is contention power due to the data waiting. $P^{comp||data}$ is different from $P^{data}$ in the aspect that the active cores also run arithmetic units that contribute to total power as $\sum_i{P^{dyn}_i(op)}$.
\begin{equation} 
\label{eq:Pcompdata}
\begin{split}
	P^{comp||data} &= P^{sta} \\
	&+ min(m,n) \times (P^{act}+ P^{LSU}+\sum_i{P^{dyn}_i(op)}) \\
	&+ max(n-m, 0) \times P^{ctn}
\end{split}
\end{equation}

\subsubsection{Model Training and Validation}
\label{sec:Validation}
This section presents the experimental results including two sets of micro-benchmarks and three application kernels (i.e. {\it matmul}, SpMV and BFS)  that are used for training and validating the models .
\paragraph{Model Training with Micro-benchmarks}
\label{sec:model-validation-micro}
Analyses of experimental results are performed based on two sets of micro-benchmarks: 22 micro-benchmarks for operation units called \emph{ unit-suite} and 9 micro-benchmarks for different operational intensities called \emph{intensity-suite}. Each micro-benchmark is executed with different numbers of SHAVE cores to measure its power consumption.
\subparagraph{Micro-benchmarks for Operation Units}
After applying the power model of operation units (Equation \ref{eq:Pfirst}) to 22 micro-benchmarks for operation units, the model-fitting percentage errors are plotted in Figure \ref{fig:OperationUnitError}. Percentage error is calculated as $PE=\frac{measurement - estimation}{measurement}$. The {\em absolute} percentage error is the absolute value of the percentage error. For this model, the absolute percentage errors are at most 6\%. Figure \ref{fig:OperationUnitError} shows the percentage error of the worst cases in all three categories: one unit, two pipe-lined units and three pipe-lined units. These results prove that the model is applicable to micro-benchmarks using either a single (e.g., performing bit wise exclusive-OR on scalar unit: SauXor) or pipe-lined arithmetic units in parallel (e.g., performing Xor on scalar and integer units, in parallel with copying from scalar to scalar unit: SauXorCmuCpssIauXor). The model also shows the compositionality of the power consumption not only for multiple SHAVE cores but also for multiple operation units within a SHAVE core.
\begin{table*}
\caption{Micro-benchmarks for Operation Units}
\label{table:Parameters}
\begin{center}
\begin{tabular*}{15cm}{ll}
\hline\noalign{\smallskip}
Description & Micro-benchmark Name \\
\noalign{\smallskip}\hline\noalign{\smallskip}
 10 micro-benchmarks using one unit                 & SAUXOR, SAUMUL, IAUXOR, IAUMUL, VAUXOR, VAUMUL, CMUCPSS,    \\
    (cf. Table 2)            &   CMUCPIVR, LSULOAD, LSUSTORE       \\ 
11 micro-benchmarks using two units    &   SAUXOR-CMUCPSS, SAUXOR-CMUCPIVR, SAUXOR-IAUMUL,  \\ 
  &   SAUXOR-IAUXOR, SAUXOR-VAUMUL, SAUXOR-VAUXOR, SAUMUL-IAUXOR,   \\ 
      & IAUXOR-VAUXOR, IAUXOR-VAUMUL, IAUXOR-CMUCPSS, LSULOAD-STORE   \\ 
1 micro-benchmarks using three-units & SAUXOR-IAUXOR-CMUCPSS \\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular*}
\end{center}
\end{table*}

\begin{figure}[!t] \centering
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Micro-benchmarks for Operational Units,
xlabel=Number of Cores,
ylabel=Percentage Error,
width=7cm, height=3.2cm,
%legend pos=outer north east,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
%symbolic x coords={0.25,0.5,1,2,4,8,16,32,64},
xtick={1,2,4,8},
%extra x tick style={xticklabel=\empty,grid=major},
ytick={-10,-5,0,5,10},
yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=NumberOfCores, y=VauXor]
{
NumberOfCores VauXor	SauXorVauXor	SauXorCmuCpssIauXor
1	3	-4	2
2	3	-5	3
4	5	-5	5
8	6	-4	5
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=NumberOfCores, y=SauXorVauXor]
{
NumberOfCores VauXor	SauXorVauXor	SauXorCmuCpssIauXor
1	3	-4	2
2	3	-5	3
4	5	-5	5
8	6	-4	5
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=NumberOfCores, y=SauXorCmuCpssIauXor]
{
NumberOfCores VauXor	SauXorVauXor	SauXorCmuCpssIauXor
1	3	-4	2
2	3	-5	3
4	5	-5	5
8	6	-4	5
};
\legend{VauXor, SauXorVauXor, SauXorCmuCpssIauXor} 
\end{axis}
\end{tikzpicture}
\caption{The upper-/ lower-bounds on percentage errors of RTHpower model-fitting for 22 micro-benchmarks shown by the worst cases of three categories: one unit (e.g., SauXor), two units (e.g., IauXorVauXor) and three units (e.g., SauXorCmuIauXor). The absolute percentage errors of micro- benchmarks for operation units are at most 6\%.}
\label{fig:OperationUnitError}
\end{figure}
\subparagraph{Micro-benchmarks for Application Intensities}
Since any application requires both computation and data movement, we design intensity-based micro-benchmarks which execute both arithmetic units (e.g., SAU) and two data transfer units (e.g., LSU0, LSU1) in a parallel manner. They are implemented with parallel instruction pipeline supported by the platform. In order to validate the RTHpower models, this micro-benchmark suite indicates different values of operation intensities (from 0.25 to 64). Operational intensity $I$ is retrieved from the assembly code by counting the number of arithmetic instructions and the number of load/store instructions. %%%%%Depending on whether computation time is longer than data transfer time, the power consumption follows either Equation \ref{eq:PalbiI} or Equation \ref{eq:PalleI} as described in Section \ref{sec:ModelEquation}.

In the models, there are platform-dependent parameters such as $\alpha$, $m$ and $P^{ctn}$. The parameter values for each application operational intensity are derived from experimental results by using Matlab function $lsqcurvefit$ . For the application intensities from 0.25 to 1, $\alpha$ is found bigger than operational intensity $I$ meaning that data transfer time is longer than computation time. The estimated power follows Equation \ref{eq:PalbiI}. For operational intensity from 2 to 64, $\alpha$ is less than $I$ meaning that data transfer time is less than computation time. The estimated power follows Equation \ref{eq:PalleI}.
We plot the model-fitting percentage errors for intensity-based micro-benchmarks in Figure \ref{fig:Intensity-Deviation}. 
%%%%%The absolute percentage errors of intensity-based micro-benchmarks are at most 7\% for the operational intensity varying from 0.25 to 64.
%as shown in Table~\ref{table:TunableParameters}

In order to obtain a  full range of estimated power with any values of intensities and numbers of cores, a fuzzy logic approach, namely Takagi Sugeno Kang (TSK) mechanism \cite{6313399}, is applied to the RTHpower models. Each intensity has a parameter set, including $\alpha$, $P^{ctn}$ and $m$. Based on the RTHpower models, each parameter set provides an individual function to estimate the power of an application based on its intensity value and a number of cores. The TSK mechanism considers the individual functions as membership functions and combines them into a general function that can be used for any input (i.e., intensity $I$ and number of cores $n$). The membership function of the fuzzy sets are triangular. After implemented the approach using Matlab Fuzzy Logic toolbox, the full range of estimated power is obtained and presented in Figure \ref{fig:TSKEstimation}. It is observed that when intensity value increases, the power scalability (i.e. the power consumption ratio of the application executed with $n$ cores to the application executed with 1 core) is also increased. The small dip in the diagram is due to the switch from Equation \ref{eq:PalbiI} to Equation \ref{eq:PalleI} at the intensity $I=2$.
\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ \includegraphics{Power_range.png}}
\caption{The power range of varied intensities and numbers of cores from RTHpower models. The dots in the figure represent measurement data.}
\label{fig:TSKEstimation}
\end{figure}

\begin{figure}[!t] \centering
%\resizebox{1\columnwidth}{!}{ \includegraphics{Intensity-Deviation.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Model-fitting Percentage Errors of Intensity-based Micro-benchmarks,
xlabel=Operational Intensity,
ylabel=Percentage Error,
width=7cm, height=3.2cm,
%legend pos=outer north east,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
%symbolic x coords={0.25,0.5,1,2,4,8,16,32,64},
xtick={1,4,8,16,32,64},
%extra x tick style={xticklabel=\empty,grid=major},
ytick={-10,-5,0,5,10},
yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=intensity, y=deviation]
{
intensity	1-core	deviation	4-cores	 6-cores	8-cores
0.25	15.15	3.46	-4.74	20.31	1.11
0.5	7.25	3.01	-3.69	13.16	0.84
1	7.75	2.56	-2.40	-7.04	0.79
2	1.37	1.78	-2.04	-2.01	0.50
4	2.72	1.44	-1.54	-1.74	0.37
8	-0.57	0.55	-0.59	35.18	0.10
16	-22.89	-1.65	5.14	89.87	-1.27
32	-22.66	0.64	4.16	98.80	-1.20
64	-18.98	7.13	-3.13	111.22	1.95
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=intensity, y=deviation]
{
intensity	1-core	2-cores	deviation	6-cores	8-cores
0.25	15.15	3.46	-4.74	20.31	1.11
0.5	7.25	3.01	-3.69	13.16	0.84
1	7.75	2.56	-2.40	-7.04	0.79
2	1.37	1.78	-2.04	-2.01	0.50
4	2.72	1.44	-1.54	-1.74	0.37
8	-0.57	0.55	-0.59	35.18	0.10
16	-22.89	-1.65	5.14	89.87	-1.27
32	-22.66	0.64	4.16	98.80	-1.20
64	-18.98	7.13	-3.13	111.22	1.95
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=intensity, y=deviation]
{
intensity	1-core	2-cores	4-cores	 6-cores	deviation
0.25	15.15	3.46	-4.74	20.31	1.11
0.5	7.25	3.01	-3.69	13.16	0.84
1	7.75	2.56	-2.40	-7.04	0.79
2	1.37	1.78	-2.04	-2.01	0.50
4	2.72	1.44	-1.54	-1.74	0.37
8	-0.57	0.55	-0.59	35.18	0.10
16	-22.89	-1.65	5.14	89.87	-1.27
32	-22.66	0.64	4.16	98.80	-1.20
64	-18.98	7.13	-3.13	111.22	1.95
};
\legend{2-cores, 4-cores, 8-cores} 
\end{axis}
\end{tikzpicture}
\caption{The absolute model-fitting percentage errors of intensity-based micro-benchmarks (operational intensity $I$ from 0.25 to 64) are at most 7\%.}
\label{fig:Intensity-Deviation}
\end{figure}
\paragraph{Model Validation with Application Kernels}
The following application kernels have been chosen to implement and validate the RTHpower models on Myriad: Dense Matrix Multiplication (a computation-intensive kernel), Sparse Matrix Vector Multiplication(a kernel with dynamic access patterns), and Breadth First Search (a data-intensive kernel of Graph500 benchmarks\cite{6114175}). All three kernels belong to the list of Berkeley dwarfs \cite{Asa06} and are able to cover the two dimensions of operational intensity and performance speed-up as shown in Figure \ref{fig:App-Cate}.
%Because the operational intensity and performance scalability are the important factors in RTHpower models and RTH framework (cf. Section \ref{sec:Framework}), the chosen kernels have varied levels of intensity and scalability values as in Figure \ref{fig:App-Cate}. 
Dense Matrix Multiplication is proved to have high intensity and scalability \cite{Ofenbeck:2014}. Sparse Matrix Vector Multiplication has low operational intensity and high speed-up due to its parallel scalability \cite{William2007}. Breadth First Search, on the other hand, has low operational intensity and saturated low scalability \cite{Cook:2013}. Since the available benchmark suites in literature are not executable on Myriad platform, the three mentioned kernels have been implemented by the authors using the Movidius Development Kit for Myriad. As the RTHpower models will be used to predict whether the RTH strategy is an energy efficient approach for an given application, we focus mainly on two settings: the 8-core setting representing the RTH strategy (i.e., using all available cores of Myriad) and the 1-core setting  representing the other extreme (i.e., using a minimum number of cores).
\begin{figure}[!t] \centering
\resizebox{0.6\columnwidth}{!}{ \includegraphics{App-Cate.png}}
\caption{Application Categories}
\label{fig:App-Cate}
\end{figure}
\subparagraph{Dense Matrix Multiplication}
Matrix multiplication ({\it matmul}) has been implemented on Myriad by using both C and assembly languages. The {\it matmul} algorithm computes matrix C based on two input matrices A and B $C=A \times B$. All three matrices in this benchmarks are stored in DDR RAM. Matrix elements are stored with float type equivalent to four bytes. The number of operations and accessed data are calculated based on matrix size $n$ as: $W=2\times n^3$ and $Q=16\times n^2$  \cite{Ofenbeck:2014}. Intensity of {\it matmul} is also varied with matrix size as: $I = \frac{W}{Q} = \frac{n}{8}$. %In our experiments, we measured power consumption of matmul with size $128 \times 128$ to $1024 \times 1024$.
The experiments are conducted until matrix size 1024x1024, the largest size that Myriad RAM memory can accommodate. Figure \ref{fig:MatmulDeviation} shows that the percentage error of {\it matmul} estimated power compared to measured power is -25\% on average for 1 core and 12\% on average for 8 cores. 

We observe that operational intensity is not enough to capture the communication pattern of the application. E.g., although a sequential version and a parallel version of a {\it matmul} algorithm have the same intensity, it is obvious that they have different communication pattern (intuitively, the sequential version doesn't have communication between cores). Since different parallel versions for different number of cores have different communication patterns (e.g., sequential version vs. 8-core version), ignoring the communication patterns contributes to the percentage errors. Therefore, we improve the models by incorporating the communication pattern $\beta$ to the models  Equation \ref{eq:Pimp1} and Equation \ref{eq:Pimp2}, where $\beta$ is computed in Equation \ref{eq:beta}. E.g., with 1 core, $\beta=\frac{1}{1-25\%}$. With 8 cores, $\beta = \frac{1}{1+12\%}$. After the improvement, the percentage errors are at most 10\% as shown in Figure \ref{fig:MatmulDeviation}. Note that communication pattern $\beta$ for each sequential/parallel version (e.g. 1-core version or 8-core version) is fixed across problem sizes and therefore it can be obtained during kernel installation and then saved as meta-data for each version in practice. 
\begin{equation} 
\label{eq:beta} 
\begin{split}
\beta = \frac{1}{1 + \overline{PE}}.
\end{split} 
\end{equation}
\begin{figure}[!t] \centering
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Dense Matrix Multiplication (matmul),
xlabel=Matrix Size,
ylabel=Percentage Error,
width=7cm, height=3.5cm,
%legend pos= outer north east,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
legend columns=2,
symbolic x coords={
128x128,
256x256,
512x512,
1024x1024,
},
x tick label style={rotate=35,anchor=east},
ytick={-20,-10,0,10,20},
yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	deviation 8-cores 1-core-after-improved 8-cores-after-improved
128x128	-31.34	2.29	-8.03	-9.50
256x256	-29.06	14.78	-4.56	2.42
512x512	-25.13	22.82	0.94	8.81
1024x1024	-17.78	20.72	9.79	7.22
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core deviation 1-core after improved 8-cores after improved
128x128	-31.34	2.29	-8.03	-9.50
256x256	-29.06	14.78	-4.56	2.42
512x512	-25.13	22.82	0.94	8.81
1024x1024	-17.78	20.72	9.79	7.22
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores deviation 8-cores-after-improved
128x128	-31.34	2.29	-8.03	-9.50
256x256	-29.06	14.78	-4.56	2.42
512x512	-25.13	22.82	0.94	8.81
1024x1024	-17.78	20.72	9.79	7.22
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores 1-core-after-improved deviation
128x128	-31.34	2.29	-8.03	-9.50
256x256	-29.06	14.78	-4.56	2.42
512x512	-25.13	22.82	0.94	8.81
1024x1024	-17.78	20.72	9.79	7.22
};
\legend{1-core-original,8-cores-original,1-core-improved,8-cores-improved} 
\end{axis}
\end{tikzpicture}
\caption{Absolute percentage errors of estimated power from measured power of {\it matmul}. After incorporating the communication patterns, the absolute percentage errors of {\it matmul} are at most 10\%.}
\label{fig:MatmulDeviation}
\end{figure}
\begin{equation} 
\label{eq:Pimp1} 
\begin{split}
	P_{improved}= (P^{comp||data} \times \frac{I}{\alpha}+  P^{data} \times \frac{\alpha-I}{\alpha}) \times \beta
\end{split} 
\end{equation}
\begin{equation} 
\label{eq:Pimp2} 
\begin{split}
	P_{improved}= (P^{comp||data} \times \frac{\alpha}{I} + P^{comp} \times \frac{I-\alpha}{I})\times \beta
\end{split} 
\end{equation}
\subparagraph{Sparse Matrix Vector Multiplication}
Sparse matrix vector multiplication (SpMV) implementation on Myriad is written in C language. All input matrix and vector of this benchmark reside in DDR RAM. This implementation uses the common data layout of SpMV which is compressed sparse row (csr) format \cite{Saad:2003}. There is no random generator supported in the RISC core so a 5 non-zero elements per row is fixed in all experiments. 
Each element of matrix and vector is stored with float type of four bytes. %Since the whole matrix is stored before performing computation in CSR format, the experiments are conducted until matrix size $2048x2048$ which is the largest that RAM memory can accommodate. 
From our implementation analysis, the number of operations and accessed data are proportional to the size of a matrix dimension $n$ as: $W=5 \times 2\times n$ and $Q=5 \times 2 \times 4 \times n$. Operational intensity of SpMV  therefore, does not depend on matrix size and is a fixed value: $I = \frac{W}{Q}= 0.25$.

Figure \ref{fig:SpMVDeviation} shows the percentage error of SpMV estimated power using Equation \ref{eq:Pimp1} and \ref{eq:Pimp2} compared to measured power. The $\beta$ values for 1-core and 8-core versions of SpMV are $\frac{1}{1 + 14\%}$ and $\frac{1}{1 - 9\%}$, respectively. The absolute percentage errors are at most 4\% as shown in Figure \ref{fig:SpMVDeviation}.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{SpMVDeviation.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Sparse Matrix Vector Multiplication,
xlabel=Matrix Size,
ylabel=Percentage Error,
width=7cm, height=3.5cm,
%legend pos= outer north east,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
legend columns=2,
symbolic x coords={32x32,
64x64,
128x128,
256x256,
512x512,
1024x1024,
%2048x2048,
},
x tick label style={rotate=35,anchor=east},
ytick={-6,-3,0,3,6},
yticklabel={\pgfmathprintnumber\tick\%}
]


\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores deviation 8-cores-after-improved
32x32	14.19	-6.25	0.83	3.32
64x64	14.19	-8.74	0.83	0.68
128x128	14.19	-9.93	0.83	-0.63
256x256	15.15	-10.32	1.66	-1.07
512x512	13.25	-7.92	0.01	1.56
1024x1024	13.25	-6.25	0.01	3.32
%2048x2048	12.32	-14.06	-0.82	-5.47
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores 1-core-after-improved deviation
32x32	14.19	-6.25	0.83	3.32
64x64	14.19	-8.74	0.83	0.68
128x128	14.19	-9.93	0.83	-0.63
256x256	15.15	-10.32	1.66	-1.07
512x512	13.25	-7.92	0.01	1.56
1024x1024	13.25	-6.25	0.01	3.32
%2048x2048	12.32	-14.06	-0.82	-5.47
};
\legend{1-core-improved,8-cores-improved} 
\end{axis}
\end{tikzpicture}
\caption{Absolute percentage errors of estimated power from measured power of SpMV. After incorporating the communication patterns, the absolute percentage errors of SpMV are at most 4\%.}
\label{fig:SpMVDeviation}
\end{figure}
\subparagraph{Breadth First Search}
We also implemente a data-intensive Graph500 kernel, namely Breadth First Search (BFS), on Myriad. BFS is the graph kernel to explore the vertices and edges of a directed graph from a starting vertex. We use the implementation of current Graph500 benchmark (omp-csr) and port it to Myriad. The output BFS graphs after running BFS implementation on Myriad are verified by the verification step of original Graph500 code to ensure the output graphs are correct.

The size of a graph is defined by its scale and edgefactor. In our experiments, we mostly use the default edgefactor of 16 from the Graph500 so that each vertex of the graph has $16$ edges in average. The graph scales are varied from 14 to 17 and the graphs has from $2^{14}$ to $2^{17}$ vertices. It is noted that graph scale 17 is the largest scale that the DDR RAM of Myriad can accommodate. From the implementation analysis, the operational intensity of BFS is a fixed value: $I = \frac{W}{Q} = 0.257$ and does not depend on edgefactor or scale. 

Figure \ref{fig:BFSDeviation} shows the percentage error of BFS estimated power using Equation \ref{eq:Pimp1} and \ref{eq:Pimp2} compared to measured power . The $\beta$ values for 1-core and 8-core versions of BFS are $\frac{1}{1+8\%}$ and $\frac{1}{1-19\%}$, respectively. The absolute percentage errors are at most 2\% as shown in Figure \ref{fig:BFSDeviation}.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{BFSDeviation.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Breadth First Search,
xlabel=Graph Scale,
ylabel=Percentage Error,
width=7cm, height=3.2cm,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
legend columns=2,
%legend pos= outer north east,
%x tick label style={rotate=45,anchor=east},
symbolic x coords={14,15,16,17},
ytick={-2,-1,0,1,2},
yticklabel={\pgfmathprintnumber\tick\%},
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=scale, y=deviation]
{
scale	deviation	8-cores-after	1-core-before	8-cores-before
14	0.59	0.29	8.81	-17.79
15	-1.75	-1.67	6.28	-19.40
16	0.59	-1.28	8.81	-19.08
17	0.59	-1.67	8.81	-19.40
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=scale, y=deviation]
{
scale	1-core-after	deviation	1-core-before	8-cores-before
14	0.59	0.29	8.81	-17.79
15	-1.75	-1.67	6.28	-19.40
16	0.59	-1.28	8.81	-19.08
17	0.59	-1.67	8.81	-19.40
};
\legend{1-core-improved,8-cores-improved} 
\end{axis}
\end{tikzpicture}
\caption{Absolute percentage errors of estimated power from measured power of BFS. After incorporating the communication patterns, the absolute percentage errors are at most 2\%.}
\label{fig:BFSDeviation}
\end{figure}
\subsubsection{Race-to-halt Prediction Framework}
\label{sec:Framework}
With the RTHpower models, we want to identify how many cores the system should use to run an application to achieve the least energy consumption. 
In order to answer the question, we need to consider the performance 
speed-up and power scalability of an application on a specific platform. 

From Amdahl's Law~\cite{4563876} the theoretical maximum speed-up of an application running on a multicore system is derived as Equation \ref{eq:Amdahl-law}, where $p$ denotes the fraction of the application that can be parallelized and $n$ is the number of cores:
\begin{equation} 
\label{eq:Amdahl-law} 
	\mbox{\it speed-up} \leq \frac{1}{(1-p)+ \frac{p}{n}}
\end{equation}
\paragraph{Framework Description}
The purpose of this framework is to identify when to and when not to use RTH for a given application. The two required inputs for making decision are power scalability and performance speed-up of the application executed with $n$ cores, where $n$ is the maximum number of cores. 
\begin{itemize}
\item Step 1: Identify meta-data, including speed-up and operational intensity, of a given application by one of the three main approaches listed: i) doing theoretical analysis to find the amount of computation work $W$, data transfer $Q$ and operational intensity $I$ as well as identify the maximum speed-up of a given application; ii) executing the application on a targeted platform (e.g., Myriad) to measure its performance speed-up and extract its operational intensity $I$; iii) using profiling tools \cite{Liu2014} to extract the number of operations $W$ and the amount of data transferred $Q$ as well as the performance speed-up of an application on a common platform (e.g., Intel platform).
\item Step 2: Compute power consumption of an application running with one core and with a maximum number of cores by the RTHpower models. Note that the RTHpower models are able to estimate power consumption for any number of cores by changing parameter n in the models. For verifying RTH strategy, we only need to apply the model for a single core and all cores. 
\item Step 3: Compare the energy consumption of the application between using 1 core and using a maximum number of cores to identify whether running a maximum number of core is the most energy-efficient.
\end{itemize}
\subsubsection{Validation}
The framework is validated with three micro-benchmarks and three application kernels. In this validation, the values of operational intensity $I$ are extracted from theoretical analysis of the implementations and performance speed-up is identified by executing the micro-benchmarks or application kernels with different numbers of cores.
\paragraph{Race-to-halt for Micro-benchmarks}
% For intensity $I=0.25$, we create three micro-benchmarks: a program with 60\% parallel code, a program with 100\% parallel code and a small-size micro-benchmarks which has high overhead. If the performance speed-up is bigger than the power ratio (namely, power scalability), RTH is an energy-saving strategy. If the performance speed-up is less than the power scalability, running with the maximum number of cores will consume more energy and race-to-halt is no longer applicable for saving energy. Figure~\ref{fig:Micro-Speed-up} shows the power scalability  of a program running $n$ cores to the program running one core for intensity 0.25. Performance speed-up for all three reported micro-benchmarks is less than the power scalability over different numbers of cores. This explains why RTH is not applicable for these three programs.
We first validate the framework with micro-benchmarks. In this validation, we measure the power scalability and performance speed-up of three micro-benchmarks: one with 60\% parallel code, one with 100\% parallel code and a small-size micro-benchmarks which has high overhead. All three micro-benchmarks have operational intensity $I=0.25$. Namely, in the micro-benchmarks, each SAUXOR instruction is followed by a LSULOAD instruction which loads 4 bytes.

All three micro-benchmarks have the same assembly code wrapped inside a loop. The number of iterations to repeat the code are the difference among them. 
We run the micro-benchmarks on one SHAVE for 1 000 000 times. If the micro-benchmark has 100\% parallel code, running it on $n$ SHAVEs requires each SHAVE performing $\frac{1}{n}$ of the amount of work (e.g.,if performing the micro-benchmark on 8 SHAVEs, each SHAVE needs to run 125 000 times). Similarly, if the micro-benchmark has a parallel fraction of 60\%, then running the program on $n$ SHAVEs requires each SHAVE to perform $(1-0.6)+(\frac{0.6}{n})$ of the amount of work (e.g.,if performing the micro-benchmark on 8 SHAVEs, each SHAVE needs to run 475 000 times). For small-size micro-benchmark, the code is executed 8 times with 1 core and once with 8 cores. Since the amount of computation is small, the relative overhead of initializing the platform and executing the small-size micro-benchmark is high. 

Figure~\ref{fig:Micro-Speed-up} shows that the power scalability of running $n$ SHAVEs to the program running 1 SHAVE varies from 1 (1 core) to 1.71 (8 cores) for operational intensity $I=0.25$. If the performance speed-up is bigger than the power scalability, RTH is an energy-saving strategy. If the speed-up is less than the power scalability, running the program with the maximum number of cores consumes more energy than running it with 1 core. When this happens, assigning one core to run the program is more energy-efficient and race-to-halt is no longer applicable for saving energy. For all three micro-benchmarks in this validation, the performance speed-up is identified by running them over different numbers of cores.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{Micro-Speed-up.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Performance and Power Scalability of Micro-benchmarks,
xlabel=Number of Cores,
%ylabel=Energy-saving Percentage,
width=7cm, height=3.2cm,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
legend columns=2,
xtick={1, 2, 4, 8},
%symbolic x coords={1,2,4,8},
%ytick={-20,-10,0,10,20},
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=powerscalability]
{
cores	powerscalability
1	1
2	1.193277311
4	1.470588235
8	1.714285714
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=speedup]
{
cores speedup 
1	1
2	0.910371319
4	1.142168675
8	1.102325581
};


\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=speedup]
{
cores speedup 
1	1
2	0.649908592
4	0.424985057
8	0.296806512
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=speedup]
{
cores speedup 
1	1
2	0.75
4	0.75
8	0.375
};

\legend{Power Scalability, Speed-up-100\%-parallel, Speed-up-60\%-parallel, Speed-up-small-size} 
\end{axis}
\end{tikzpicture}
\caption{Performance and power scalability of micro-benchmarks with operational intensity $I=0.25$. All three reported micro-benchmarks have performance speed-up less than platform power scalability.}
\label{fig:Micro-Speed-up}
\end{figure}
The energy consumption of the three micro-benchmarks is shown in Figure \ref{fig:Micro-Energy}. All three micro-benchmarks achieve the least energy consumption when executed with one core, from both measured and estimated data. The model estimation and actual measurement show that RTH is not applicable to the three micro-benchmarks.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{Micro-Energy.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Energy Consumption of Micro-benchmarks,
xlabel=Number of Cores,
ylabel=Energy (mJ),
width=7cm, height=3.2cm,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
legend columns=2,
%symbolic x coords={1, 2, 4, 8},
xtick={1, 2, 4, 8},
%x tick label style={rotate=35,anchor=east},
%ytick={-20,-10,0,10,20},
%yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	169.218
2	221.804
4	217.875
8	263.16

};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	194.8528068
2	229.4848075
4	207.5381265
8	266.0719045
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	169.218
2	310.696
4	585.55
8	977.364
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	194.8528068
2	321.4550312
4	557.7691334
8	988.1786779
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	342
2	500
4	600
8	1616
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	357
2	568
4	700
8	1632
};

\legend{100\%-parallel-measurement,100\%-parallel-estimation,60\%-parallel-measurement,60\%-parallel-estimation, small-size-measurement,small-size-estimation} 
\end{axis}
\end{tikzpicture}
\caption{Energy consumption of micro-benchmarks with operational intensity $I=0.25$.
For all three reported micro-benchmarks, the programs executed with 1 core consume the least energy, compared to 2, 4, 8 cores, from both measured data and estimated data.}
\label{fig:Micro-Energy}
\end{figure}
\paragraph{Race-to-halt for Dense Matrix Multiplication}
The {\it matmul} application has increasing values of operational intensity over input sizes and its performance speed-up is higher than its power scalability on Myriad. 
Therefore, running {\it matmul} with the 8 cores is more energy-efficient than running it with one core. Figure ~\ref{fig:Matmul-RTH} shows how many percentages of energy-saving if executing {\it matmul} with 8 cores instead of 1 core, from both measured and estimated data. The energy saving percentage is computed based on the energy gap of running 1 core and 8 cores divided by energy consumed by running 1 core as in Equation \ref{eq:ES}.
\begin{equation} 
\label{eq:ES} 
	 ES = \frac{E^{1core} - E^{8cores}}{E^{1core}}
\end{equation}
The framework can predict that RTH should be applied to {\it matmul} over different matrix sizes. By using RTH for {\it matmul}, we can save from 20\% to 61\% of {\it matmul} energy consumption. RTH is a good strategy for {\it matmul}. We observe that the energy saving reduces when matrix size increases due to the decrease of performance speed-up from size $128x128$. The reason is that a matrix size bigger than $128x128$ makes the data set no longer fit in the last level cache (or L2 cache of 64KB) and thereby lowers performance (in flops).  
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{SpMV-RTH.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Matmul Energy-saving by Race-to-halt,
xlabel=Matrix Size,
ylabel=Energy-saving Percentage,
width=6cm, height=3.5cm,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
symbolic x coords={
128x128,
256x256,
512x512,
},
x tick label style={rotate=35,anchor=east},
%ytick={-20,-10,0,10,20},
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
128x128	60.73 0
256x256	25.33 1
512x512	19.91 0
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
128x128	60.20 0
256x256	30.32 1
512x512	26.28 0
};

\legend{Measurement, Model Estimation} 
\end{axis}
\end{tikzpicture}
\caption{{\it matmul} Energy-saving by Race-to-halt. This diagram shows how many percentages of energy-saving if execute {\it matmul} with 8 cores instead of 1 core. Since the energy-saving percentage is positive over different matrix sizes, RTH is a energy-saving strategy for {\it matmul}. Energy-saving percentage from model estimation for {\it matmul} has standard deviation less than 3\%.}
\label{fig:Matmul-RTH}
\end{figure}
\paragraph{Race-to-halt for Sparse Matrix Vector Multiplication}
SpMV has a fixed value of operational intensity over input sizes. From the RTHpower models as well as measurement data, the power scalability of SpMV is relatively constant. However, SpMV has performance speed-up higher than its power scalability. 
Therefore, running SpMV with the maximum number of cores is more energy-efficient than running it with one core. Figure ~\ref{fig:SpMV-RTH} shows how many percentages of energy-saving if executing SpMV with 8 cores instead of 1 core, from both measured and estimated data. The framework can predict that RTH should be applied to SpMV over different matrix sizes. By using RTH for SpMV, we can save from 45\% to 59\% of SpMV energy consumption. RTH is a good strategy for SpMV.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{SpMV-RTH.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=SpMV Energy-saving by Race-to-halt,
xlabel=Matrix Size,
ylabel=Energy-saving Percentage,
width=8cm, height=3.5cm,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
symbolic x coords={32x32,
64x64,
128x128,
256x256,
512x512,
1024x1024,
%2048x2048,
},
x tick label style={rotate=35,anchor=east},
%ytick={-20,-10,0,10,20},
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
32x32	46.46	0.00
64x64	53.76	0.98
128x128	59.28	0.55
256x256	58.14	3.00
512x512	55.46	1.66
1024x1024	49.06	1.34
%2048x2048	59.54	0.56
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
32x32	44.99	0.00
64x64	53.75	0.98
128x128	59.81	0.56
256x256	59.21	3.05
512x512	54.68	1.63
1024x1024	47.22	1.29
%2048x2048	61.26	0.58

};

\legend{Measurement, Model Estimation} 
\end{axis}
\end{tikzpicture}
\caption{SpMV Energy-saving by Race-to-halt. This diagram shows how many percentages of energy-saving if execute SpMV with 8 cores instead of 1 core. Since the energy-saving percentage is positive over different matrix sizes, RTH is a energy-saving strategy for SpMV.}
\label{fig:SpMV-RTH}
\end{figure}
\paragraph{Race-to-halt for Breadth First Search}
In our set of application kernels implemented on Myriad, 
BFS is the application kernel able to prove that running with a
maximum number of cores does not always give the least energy consumption. From both measured data and estimated data, the total energy consumed by running with one core is less than the total energy by running with 8 cores at scale 16 and 17. There are negative values of -5\% and -3\% in Figure~\ref{fig:BFS-RTH} if running BFS with 8 cores instead of 1 cores at scale 16 and 17, respectively. The RTHpower models can predict when to apply RTH precisely for different scales. 
%The models show that RTH should be applied on scale 14 and 15 while it should not be applied on scale 16 and 17. 

The result can be explained by the relation between BFS power scalability and performance speed-up. Since BFS has a fixed value of operational intensities across graph scale, from RTHpower models (cf. Equation \ref{eq:Pimp1} and \ref{eq:Pimp2}), it is understood that BFS power consumption does not depend on graph scales and its power scalability is a fixed value. From the measurement results, we also observe that BFS power-scalability is relatively constant over the graph scales. However, BFS speed-up in our experiments decreases when scale increases. The reason is that with the same graph degree, when scale increases, the graph becomes more sparse and disconnected. Compared to the Graph500 implementation, BFS search on Myriad are performed from a chosen subset of source nodes. The speed-up then, becomes less than power scalability at scale 16 and 17. Therefore, running BFS with 8 cores at bigger graph scales (i.e., 16 and 17 in our experiments) consumes more energy than running BFS with one core.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{BFS-RTH.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=BFS Energy-saving by Race-to-halt,
xlabel=Graph Scale,
ylabel=Energy-saving Percentage,
width=7cm, height=3.2cm,
legend style={at={(0.5,-0.5)},
anchor=north,legend columns=-1},
%symbolic x coords={14,15,16,17},
xtick=data,
%x tick label style={rotate=35,anchor=east},
%ytick={-20,-10,0,10,20},
minor ytick={0},grid=minor,
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
14	23.45	0.66
15	11.29	0.30
16	-5.82	-0.06
17	-3.30	-0.04
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
14	23.68 0
15	11.21 0
16	-3.86 0
17	-0.98 0

};

\legend{Measurement,Model Estimation} 
\end{axis}
\end{tikzpicture}
\caption{BFS Energy-saving by Race-to-halt. This diagram shows how many percentages of energy-saving if executing BFS with 8 cores instead of 1 core. The positive percentages at scale 14 and 15 mean that RTH should be applied. The negative percentages at scale 16 and 17 mean that RTH should not be applied. The standard deviation of BFS energy-saving percentage is less than 3\%, from scale 14 to 17.}
\label{fig:BFS-RTH}
\end{figure}
\subsubsection{Conclusion}
In this study, new fine-grained power models have been proposed to provide insights into how a given application consumes energy when executing on an ultra-low power embedded system. In the models, applications are represented by their operational intensity. The models have been validated on Movidius Myriad, an ultra-low power embedded platform. Experimental results on 31 micro-benchmarks and three application kernels have shown high accuracy of estimated data by the model. %We have also shown that by using the models, we can predict whether RTH is energy-efficient for an application. We presented real scenarios when to use RTH and when not to use RTH and the framework based on the models could predict the scenarios precisely.
Based on the models, we have devised a new framework to predict whether RTH is applicable to a given application. The framework has been validated by both micro-benchmarks and real application kernels, showing precise prediction. Improving and applying the models and framework to other embedded platforms (e.g. ARM) and application kernels (e.g. other Berkeley dwarfs) are parts of our future work.    
